Engagement and Disclosures in LLM-Powered Cognitive Behavioral Therapy Exercises: A Factorial Design Comparing the Influence of a Robot vs. Chatbot Over Time

Many researchers are working to address the worldwide mental health crisis by developing therapeutic technologies that increase the accessibility of care, including leveraging large language model (LLM) capabilities in chatbots and socially assistive robots (SARs) used for therapeutic applications. Yet, the effects of these technologies over time remain unexplored. In this study, we use a factorial design to assess the impact of embodiment and time spent engaging in therapeutic exercises on participant disclosures. We assessed transcripts gathered from a two-week study in which 26 university student participants completed daily interactive Cognitive Behavioral Therapy (CBT) exercises in their residences using either an LLM-powered SAR or a disembodied chatbot. We evaluated the levels of active engagement and high intimacy of their disclosures (opinions, judgments, and emotions) during each session and over time. Our findings show significant interactions between time and embodiment for both outcome measures: participant engagement and intimacy increased over time in the physical robot condition, while both measures decreased in the chatbot condition.

==> Appendices.tex <==
\section{GPT-3.5 Parameters} \label{gpt-parameters}
The input parameters for OpenAI’s chat completion API were:\\
\renewcommand{\thetable}{S1}
\begin{table}[H]
\centering
\begin{tabular}{|l|l|}
\hline
model & gpt-3.5-turbo \\ \hline
messages & <transcript> \\ \hline
stop & Patient \\ \hline
temperature & 1 \\ \hline
frequency\_penalty & 2 \\ \hline
presence\_penalty & 2 \\ \hline
n & 2 \\ \hline
max\_tokens & 150 \\ \hline
\end{tabular}
\caption{\textbf{LLM Parameters.} Model parameters for OpenAI's completion API.}
\label{tab:model_parameters}
\end{table}
The transcript being sent includes all of the previous messages and the user's latest message.

For moderator, the input parameters were same as above, except the temperature was increased to 2 and the values for n and max\_tokens were not sent.

\section{Python Libraries} \label{python-libraries}
\renewcommand{\thetable}{S2}
\begin{table}[H]
\centering
\begin{tabular}{|l|l|}
\hline
pandas & 2.0.2 \\ \hline
matplotlib & 3.7.1 \\ \hline
scipy & 1.10.1 \\ \hline
pingouin & 0.5.3 \\ \hline
numpy & 1.24.3 \\ \hline
\end{tabular}
\caption{\textbf{Python libraries.} The Python libraries used during our analysis and data cleaning.}
\label{tab:python}
\end{table}

\section{R Packages} \label{rpackages}

\begin{table}[H]
\centering
\renewcommand{\thetable}{S3}
\begin{tabular}{|l|l|}
\hline
readxl & 1.4.2 \\ \hline
dplyr & 1.1.2 \\ \hline
tidyr & 1.3.0 \\ \hline
outliers & 0.15 \\ \hline
rstatix & 0.7.2 \\ \hline
ggpubr & 0.6.0 \\ \hline
car & 3.1-2 \\ \hline
lmtest & 0.9-40 \\ \hline
DescTools & 0.99.49 \\ \hline
ggplot2 & 3.4.2 \\ \hline
ggcorrplot & 0.1.4 \\ \hline
MASS & 7.3-60 \\ \hline
afex & 1.3-0 \\ \hline
pastecs & 1.4.2 \\ \hline
ez & 4.4-0 \\ \hline
reshape & 0.8.9 \\ \hline
\end{tabular}
\caption{\textbf{R packages.} The R packages used during our statistical analysis.}
\label{tab:r}
\end{table}


==> Privacy_and_Ethics.tex <==
Extensive measures were taken to protect study participant safety and privacy. In the consent procedure, all participants were informed that an LLM was used for dialog and all agreed to proceed. Participants received randomly generated usernames and passwords to access the online platform; no identifiable information was collected and shared with the LLM.
%unless they chose to disclose it during the conversation. 
Our prompts contained no demographic information to avoid LLMs' inherent biases to the greatest extent possible. The collected data were stored securely on AWS S3 storage during the study and were later moved to OneDrive. Both cloud services were approved by our University's IRB and were only accessible by IRB-approved researchers on the team. We screened out participants with moderately severe depression to prevent potential harm caused by the sensitive CBT context. We provided participants with our University's mental health crisis hotline number on the platform at every interaction. Participants were encouraged to contact researchers for help if needed at any point. 
